A temporal logic approach to modular design of synthetic biological circuits

We present a new approach for the design of a synthetic biological circuit whose behaviour is specified in terms of signal temporal logic (STL) formulae. We first show how to characterise with STL formulae the input/output behaviour of biological modules miming the classical logical gates (AND, NOT, OR). Hence, we provide the regions of the parameter space for which these specifications are satisfied. Given a STL specification of the target circuit to be designed and the networks of its constituent components, we propose a methodology to constrain the behaviour of each module, then identifying the subset of the parameter space in which those constraints are satisfied, providing also a measure of the robustness for the target circuit design. This approach, which leverages recent results on the quantitative semantics of Signal Temporal Logic, is illustrated by synthesising a biological implementation of an half-adder.

==> algo.tex <==
% !TEX root =  ModulesSysBio.tex

\section{Parameter Synthesis}
\label{sec:algo}

{\bf Describe how we do parameter synthesis exploiting modularity, and why this is a cool idea.

 Present the algorithm taking the intersection of validity domains, the idea of exploiting validity of edge compatibility formulae, how we obtain the final/target property by local analysis, how we deal with input signals to preserve modularity. 
 
  It would be nice to have a theorem here, stating that if we pick a parameter configuration in the intersection of the validity domains, the target property is true. The story about the input can make this 
more difficult than expected.}

Given a network of modules $\Gamma=(\mathcal{M},\mathcal{N}, \mathcal{E}, P_{Target})$, our goal is to find the validity domain of each free parameters of $\Gamma$ s.t. $\Gamma \models \mathcal{P}_{Target}$, where $\mathcal{P}_{Target}=PT_{1} \wedge \cdots \wedge PT_{m}$.
If we call $\mathcal{K}_{\Gamma}=K_{p_{1}} \times \cdots \times K_{p_{n}}$ the iperbox of all real limited intervals specifying the admissible values of all free parameters of $\Gamma$,  $\Gamma \models P_{Target}$ if and only if the validity domain of each box $ K_{p_{i}}$ is different from the empty set.  As said in the last section, we want solve this problem exploiting the modularity of the network. 

Let  $S$ a dynamic systems and $P$ a QMiTL formula (a property), then  we note 
$$\mbox{Check}(S, P, \mathcal{K}_{\Gamma})=A_{p_{1}} \times \cdots \times A_{p_{n}},$$
where $$A_{i}=\begin{cases} 
\mbox{the validity domain of } K_{p_{i}} \mbox{ if } p_{i} \mbox{ is a free parameter of } S \mbox{ or } P \\
K_{p_{i}} \qquad \mbox{otherwise}\\
\end{cases}$$

Let $\mathcal{V}_{1},...,\mathcal{V}_{r}$ a set of validity domains, where each $\mathcal{V}_{i} ={Check}(S, P, \mathcal{K}_{\Gamma})$ for some $S,P$ and $\mathcal{K}_{\Gamma}$. Then we note
$$\mbox{InterCheck}(\mathcal{V}_{1},...V_{r})= \mbox{ the intersection of all the validity domains}. $$

Let $\Omega=( \mathcal{P}_{Head},\mathcal{P}_{Module}, \mathcal{P}_{Junction}  )$ the network property set of the module.

\begin{algorithmic}[1]
 \STATE   $\Gamma,\mathcal{K}_{\Gamma}, \Omega$
 \FOR {$ z=1,...m$}
     \FOR{$\forall P \in \mathcal{P}_{Head}$ s.t. $P$ is a subset of an input property of $PT_{j}$ }
 \STATE{ $A_{p_{1}} \times \cdots \times A_{p_{n}}$=Check($M_{Head},P, K_{p_{1}} \times \cdots \times K_{p_{n}}$)}
        \STATE  j=1
    \STATE $A_{j}=A_{p_{1}} \times \cdots \times A_{p_{n}}$
    \STATE j=j+1
    \ENDFOR
     \STATE $A_{p_{1}} \times \cdots \times A_{p_{n}}=\mbox{InterCheck}(A_{1},...,A_{\mbox{lenght} (\mathcal{P}_{Head})})$.    
   
 \FOR {$i=1,...,n$}
 \STATE $ B_{p_{i}}=K_{p_{i}}$
 \ENDFOR
 \FOR{$\forall M \in \mathcal{M}$ }
   \FOR{$\forall P \in \mathcal{P}_{M}$ }
    \STATE{ $B_{p_{1}} \times \cdots \times B_{p_{n}}$=Check($M,P, B_{p_{1}} \times \cdots \times B_{p_{n}}$)}
    \STATE  j=1
    \STATE $B_{j}=B_{p_{1}} \times \cdots \times B_{p_{n}}$
    \STATE j=j+1
    \ENDFOR
     \STATE $B_{p_{1}} \times \cdots \times B_{p_{n}}=\mbox{InterCheck}(B_{1},...,B_{\mbox{lenght} (\mathcal{P}_{M})})$.    
        \ENDFOR
 
    \FOR{$\forall P=\{\varphi_{O} \rightarrow \varphi_{I}\} \in \mathcal{P}_{Junction}$ }
    \STATE $\varphi_{O}=\varphi_{{I_{prototype}}}$
 \STATE{ $C_{p_{1}} \times \cdots \times C_{p_{n}}$=Check($M_{incoming},\varphi_{O}, C_{p_{1}} \times \cdots \times C_{p_{n}}$)}
    \ENDFOR   
  \STATE $D_{p_{1}} \times \cdots \times D_{p_{n}}=\mbox{InterCheck}(A_{p_{1}} \times \cdots \times A_{p_{n}},B_{p_{1}} \times \cdots \times B_{p_{n}},C_{p_{1}} \times \cdots \times C_{p_{n}})$.
        \STATE $D_{z}=D_{p_{1}} \times \cdots \times D_{p_{n}}$
      \ENDFOR
      
       
  \STATE $E_{p_{1}} \times \cdots \times E_{p_{n}}=\mbox{InterCheck}(D_{1}, ..., D_{m})$.
    \FOR {$\forall i $} 
   \IF{$E_{p_{i}} = \emptyset$}  \PRINT  No solution
     \STATE Stop
     \ENDIF
      \ENDFOR
       \RETURN  $E_{p_{1}} \times \cdots \times E_{p_{n}}$ 
      

\end{algorithmic}








==> modules.tex <==
% !TEX root =  ModulesSysBio.tex

\section{Logical characterisation of modules}
\label{sec:modules}

{\bf Define a module, explain how we characterise it logically from a behavioural point of view. Show an example (a gate ).}

Our modules, intuitively,  are small biological networks (with a small number of nodes) that, ``in particular situations", demonstrate ``specific behaviours", i.e., for some values of their parameters, the module satisfies a set of specific temporal properties. We will give now the formal definition of them.

Recall that  the dynamics of the network is described by a set of ODE such as:
$$  
\frac {d x_{i}}{dt} =\sum^{m}_{i=1} S_{ij} f_{j}(x_{1},...,x_{n},h_{1},...h_{r}),  \qquad \mbox{ }n=1,...,n,
$$

where  $S$ is the stochiometric matrix, $f:\mathbb{R}^{n+s} \rightarrow \mathbb{R}$ is the rate function associated with the $j_{th}$ reaction of a module with $n$ biochemical species, ${\bf x}=(x_{1},...,x_{n})$ is the concentration vector and $h_{1},...h_{r}$ are the free parameters of the module. %s.t. each $h_{i} \in K_{h_{i}}$, with $ K_{h_{i}}$ limited real interval.

%Our graphical representation of the module is a signed oriented graph $(\mathcal{G},\mathcal{A},s)$ whose set of vertices $\mathcal{G}$ includes all the molecules in the model and whose arcs are labelled by the Jacobian of the vector field $f$. An arc connects a pair of vertices $(i,j)\in \mathcal{A}$  iff  $\frac{\partial f_{i}}{\partial x_{i}}\neq0$. Finally,  the sign function, describing the direction of the interaction is defined as $s(i,j)=sgn\frac{\partial f_{i}}{\partial x_{i}}$, \cite{Rad}.

For the type of study that we want do, we can treat the modules as a {\it black-box}, with a certain number of input variables and a certain number of output variables, related in some way, i.e. the non-linear temporal dynamics of a module can be described by a set of input and output trajectories. 

The module may need external signals to activate its dynamics. Alternatively,  the production of its constituent can start independently.  
%We call {\it Input $I$ of a module} each node $j \in \mathcal{G}$ that doesn't have an incoming edge, i.e. s.t. $  (i,j) \notin \mathcal {A}$ for $\forall i \in \mathcal{G} \setminus \{j\}$ and  we denote by $x_{I}: [0, T] \rightarrow \mathbb{R}$ the {\it input signal trajectory} (the variation of the signal's concentration over time). At the same time, the species produced by the module will be considered as  {\it Outputs} signals $O$    with no outgoing edge, i.e. s.t. $  (i,j) \notin \mathcal {A}$ for $\forall j \in \mathcal{G} \setminus \{i\}$, or with edge that forms a cycle with one ore more other nodes, i.e. s.t. $ \exists j \in \mathcal{G}: (i,j)\in  \mathcal {A}$ and  $(j,i) \in \mathcal {A}$ and we call $ x_{O}:[0,T] \rightarrow \mathbb{R}$ the output signal's trajectory.
We call {\it Input} $I$ of a module each signal needed to activate the dynamics. If the production of its constituent can start independently we say that the module has no input signals;  we denote by $x_{I}: [0, T] \rightarrow \mathbb{R}$ the {\it input signal trajectory} (the variation of the signal's concentration over time).  
At the same time, we call {\it Outputs $O$  of a module} each node  produced  by the module that it will be investigated (studied). We call $ x_{O}$ {\it the output signal's trajectory}. 


  A {\it behaviour} of the module is a set of trajectories described by a logic formula. If $I$ is an input signal, we call $\varphi_{I}(\omega_{1},..., \omega_{s})$ the logic formula that describes the behaviour of $I$; similarly, if $O$ is an output signal, we call $\varphi_{O}(\omega_{1},..., \omega_{s})$ a logic formula that describes the behaviour of $O$, where $\omega_{1},..., \omega_{s}$ are the free parameters of all logic formulae of the module, as, for example, the  starting time of the signal, or the duration of the signal or its height. %and we have that each $\omega_{i} \in K_{\omega_{i}}$, with $K_{\omega_{i}}$ limited real interval.

We can now characterize a behaviour of the whole module seen as a black box. Let  $I_{1},...,I_{m}$ be all the input nodes and $O_{1},...,O_{q}$ be all the output nodes, and let $\mathcal{F}_{ \mathcal{I}}$  denotes a set of formulae describing the behaviours of the inputs $ I_{1},...,I_{m}$ and  $\mathcal{F}_{ \mathcal{O}}$  denotes a set of formulae describing the behaviours of the outputs $ O_{1},...,O_{q}$. 
 
A  {\it temporal property of the module} is an implication formula: 
\begin{equation}
 \varphi_{I_{1}} \wedge...\wedge \varphi_{I_{s}}  \rightarrow  \varphi_{O_{1}} \wedge...\wedge \varphi_{O_{r}} ,
 \label{temporalproperty}
 \end{equation}
  where $\{ \varphi_{I_{1}},...,\varphi_{I_{s}} \}$ is a subset of $\mathcal{F}_{ \mathcal{I}}$ and $\{ \varphi_{O_{1}},...\varphi_{O_{r}} \}$ is a subset of $\mathcal{F}_{ \mathcal{O}}$.
  Note that it is possible to have more than one temporal property for each module.

%For notational simplicity, we equivalently denote the previous formula as:   $$\{ \psi_{I_{1}},...,\psi_{I_{s}} \} \rightarrow \{ \psi_{O_{1}},...\psi_{O_{r}} \}.$$
  
We can now give the definition module.

\begin{definition}{(\bf Module)} A {\it module} $M$ is a tuple $(\mathcal{S}, \mathcal{I}, \mathcal{O},\mathcal{F}_{ \mathcal{I}},\mathcal{F}_{ \mathcal{O}}, \mathcal{P},  \mathcal{K}_{free})$ where:
\begin{itemize}
  \item $\mathcal{S}$ is the set of ODEs:$$  
\frac {d x_{i}}{dt} =\sum^{m}_{i=1} S_{ij} f_{j}(x_{1},...,x_{n},h_{1},...,h_{r}),  \qquad \mbox{ }n=1,...,n,
$$describing the dynamics of the module;
  \item $\mathcal{I}=\{I_{1},...,I_{m}\}$ is the set of all input signals;
  \item $\mathcal{O}=\{ O_{1},...,O_{q} \}$ is the set of all output signals;
  \item $\mathcal{F}_{ \mathcal{I}}=\{ \varphi_{I_{1}}(\omega_{1},..., \omega_{s}),...,\varphi_{I_{m}}(\omega_{1},..., \omega_{s}) \}$  is the set of all input signal behaviours;
  \item $\mathcal{F}_{ \mathcal{O}}=\{ \varphi_{O_{1}} (\omega_{1},..., \omega_{s}),...\varphi_{O_{q}} (\omega_{1},..., \omega_{s})\}$  is the set of all output signal; behaviours,
  \item $\mathcal{P}=\{ P_{1},...P_{v} \}$  is the set of the properties, with each $P_{i}$ of the form given by (\ref{temporalproperty}),
 %   \item $ \mathcal{K}_{fixed}=(k_{1},...k_{m})$ is the set of value of all fixed parameters of the module and the properties;
  \item $ \mathcal{K}_{free}=(K_{h_{1}},...K_{h_{r}},K_{\omega_{1}},...K_{\omega_{s}})$, where, for $\forall i=1,...r$, $K_{h_{i}}$ is a limited real interval specifying the admissible values of the free parameter $h_{i}$ and,  for $\forall i=1,...s$, $K_{\omega_{i}}$ is a limited real interval specifying the admissible values of the free parameter $\omega_{i}$.
\end{itemize}
\end{definition}

COMMENTO: problema define i metaparametri forse aggiungere alla tupla del modulo un $\mathcal{K}_{meta}$ where each  $h \in \mathcal{K}_{meta} $ is of the type $h=\{ h_{high}, h_{low}\}$ or $h=\{1,0\}$.

\begin{example}[AND logic gate]
To better understand this concept we give an example.
Consider the AND logic gate ...

 The 3-ODE model is as follows:
$$
\begin{cases} 
\frac {dx_{A}}{dt} =  b_{A} \cdot s_{1} - d_{A} \cdot x_{A}  \\
\frac {dx_{B}}{dt} =  b_{B} \cdot s_{2} - d_{B} \cdot x_{B} \\
\frac {dx_{C}}{dt} =  b_{C} \cdot \frac{ {x_{A}}^{n}}{K_{AC}^{n}+{x_{A}}^{n}}  \cdot  \frac{  {x_{B}}^{n}}{K_{BC}^{n}+{x_{B}}^{n}}  - dc \cdot x_{C},
\end{cases}
$$
where $x_{A}$ is the concentration of the protein A, $s_{1}$ is the signal that activates the production of $A$, $K_{AB}$ and  $K_{BC}$ are  the concentration thresholds  of $A$ and $B$ to activate the production of $C$.

The trajectory obtained with these values is shown in Figure ~\ref{traj_AND}. 
\begin{figure}
\centering
\subfigure[Traj AND 00: with $x_{A}(0)=1, s_{1}=0, x_{B}(0)=1, s_{2}=0$]{\label{fig:AND00}{\includegraphics[width=0.45\textwidth]{./figs/traj_AND_00.eps}}}
\subfigure[Traj AND 01: with $x_{A}(0)=1, s_{1}=0, x_{B}(0)=0, s_{2}=1$]{\label{fig:AND01}{\includegraphics[width=0.45\textwidth]{./figs/traj_AND_01.eps}}}
\subfigure[Traj AND 10: with $x_{A}(0)=0, s_{1}=1, x_{B}(0)=1, s_{2}=0$]{\label{fig:AND10}{\includegraphics[width=0.45\textwidth]{./figs/traj_AND_10.eps}}}
\subfigure[Traj AND 11: with $x_{A}(0)=0, s_{1}=1, x_{B}(0)=0, s_{2}=1$]{\label{fig:AND11}{\includegraphics[width=0.45\textwidth]{./figs/traj_AND_11.eps}}}
\caption{The trajectories of the 3-ODE model of the AND gate varying the initial concentration of $A$ and $B$ and the signals $s_{1}$ and $s_{2}$, with
$x_{C}(0)=0, b_{A}=1, d_{A}=1, K_{AC}=0.5, b_{B}=1, d_{B}=1, K_{BC}=0.5, b_{C}=1, d_{C}=1 $ and $ n=15.$}
\label{traj_AND}
\end{figure}

The property described above, in terms of STL, is:
%{\bf Properties}:
\begin{description}
  \item[ $pA_{high}$:]$ x_{A}[t]> xAh$
  \item[ $pA_{low}$:]$ x_{A}[t]< xAl$
    \item[ $pB_{high}$:]$ x_{B}[t]> xBh$
  \item[ $pB_{low}$:]$ x_{B}[t]< xBl$
    \item[ $pC_{high}$:]$ x_{C}[t]> xCh$
  \item[ $pC_{low}$:]$ x_{C}[t]< xCl$
  \item[ $\varphi_{1}$:]$ (G_{[0,\delta_{1}]}(pA_{low} \wedge pB_{low}))\rightarrow F_{[0, t_{1}]}(G_{[0,\delta_{2}]}(pC_{low}))$
\item[ $\varphi_{2}$:]$ (G_{[0,\delta_{1}]}(pA_{low} \wedge pB_{high}))\rightarrow F_{[0, t_{1}]}(G_{[0,\delta_{2}]}(pC_{low}))$
\item[ $\varphi_{3}$:]$ (G_{[0,\delta_{1}]}(pA_{high} \wedge pB_{low}))\rightarrow F_{[0, t_{1}]}(G_{[0,\delta_{2}]}(pC_{low}))$
\item[ $\varphi_{4}$:]$ (G_{[0,\delta_{1}]}(pA_{high} \wedge pB_{high}))\rightarrow F_{[0, t_{1}]}(G_{[0,\delta_{2}]}(pC_{high}))$
\end{description}

\begin{tabular}{ |c|c|c| }
\hline
\multicolumn{2}{|c|}{\textbf{Inputs}} & \multicolumn{1}{|c|}{\textbf{Output}} \\
\hline
\multicolumn{2}{|c|}{} & \multicolumn{1}{|c|}{max delay=$t_1 - \delta_2 $} \\
\hline
\multicolumn{2}{|c|}{duration=$\delta_1$} & \multicolumn{1}{|c|}{min. duration=$\delta_2 $} \\
\hline
  \textbf{pA} & \textbf{pB} & \textbf{pC}\\
\hline
  low & low & low\\
\hline
  low & high &  low \\
\hline 
 high & low & low\\
\hline 
 high & high & high \\
  \hline
\end{tabular}

\begin{tabular}{ |c|c|c|c| }
\hline
\multicolumn{2}{|c|}{\textbf{Inputs}} & \multicolumn{2}{|c|}{\textbf{Output}} \\
\hline
\multicolumn{2}{|c|}{} & \multicolumn{2}{|c|}{max delay=$t_1 - \delta_2 $} \\
\hline
\multicolumn{2}{|c|}{duration=$\delta_1$} & \multicolumn{2}{|c|}{min. duration=$\delta_2 $} \\
\hline
  \textbf{pA} & \textbf{pB} & \textbf{pC} &\\
\hline
  low & low & low & \\
\hline
  low & high &  low & \\
\hline 
 high & low & low & \\
\hline 
 high & high & high & \\
  \hline
\end{tabular}



\end{example}







